The Completed SDSS-IV extended Baryon Oscillation Spectroscopic Survey: Cosmological Implications from two Decades of Spectroscopic Surveys at the Apache Point observatory

We present the cosmological implications from final measurements of clustering using galaxies, quasars, and Ly$\alpha$ forests from the completed Sloan Digital Sky Survey (SDSS) lineage of experiments in large-scale structure. These experiments, composed of data from SDSS, SDSS-II, BOSS, and eBOSS, offer independent measurements of baryon acoustic oscillation (BAO) measurements of angular-diameter distances and Hubble distances relative to the sound horizon, $r_d$, from eight different samples and six measurements of the growth rate parameter, $f\sigma_8$, from redshift-space distortions (RSD). This composite sample is the most constraining of its kind and allows us to perform a comprehensive assessment of the cosmological model after two decades of dedicated spectroscopic observation. We show that the BAO data alone are able to rule out dark-energy-free models at more than eight standard deviations in an extension to the flat, $\Lambda$CDM model that allows for curvature. When combined with Planck Cosmic Microwave Background (CMB) measurements of temperature and polarization the BAO data provide nearly an order of magnitude improvement on curvature constraints. The RSD measurements indicate a growth rate that is consistent with predictions from Planck primary data and with General Relativity. When combining the results of SDSS BAO and RSD with external data, all multiple-parameter extensions remain consistent with a $\Lambda$CDM model. Regardless of cosmological model, the precision on $\Omega_\Lambda$, $H_0$, and $\sigma_8$, remains at roughly 1\%, showing changes of less than 0.6\% in the central values between models. The inverse distance ladder measurement under a o$w_0w_a$CDM yields $H_0= 68.20 \pm 0.81 \, \rm km\, s^{-1} Mpc^{-1}$, remaining in tension with several direct determination methods. (abridged)

==> astromacro.tex <==
\usepackage{color}
\usepackage{graphicx}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lyman series lines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ly}{Lyman}
\newcommand{\Lya}{\mbox{Ly$\alpha$}}
\newcommand{\lya}{\mbox{Ly$\alpha$}}
\newcommand{\lyb}{\mbox{Ly$\beta$}}
\newcommand{\lyg}{\mbox{Ly$\gamma$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kms}{\mbox{km s$^{-1}$}}
\newcommand{\cmm}{\mbox{cm$^{-2}$}}
\newcommand{\cmmm}{\mbox{cm$^{-3}$}}
\newcommand{\escsh}{$\mathrm{ergs}
        \mathrm{\ s}^{-1}
        \mathrm{\ cm}^{-2}
        \mathrm{\ sr}^{-1}
        \mathrm{\ Hz}^{-1}$}
\newcommand{\hmpc}{\mbox{$h^{-1}$Mpc}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Light elements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\het}{\mbox{$^3$He}}
\newcommand{\hef}{\mbox{$^4$He}}
\newcommand{\lisv}{\mbox{$^7$Li}}
\newcommand{\lisx}{\mbox{$^6$Li}}
\newcommand{\yp}{\mbox{Y$_p$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cosmological  Parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ETA}{\mbox{$\eta $}}
\newcommand{\ob}{\mbox{$\Omega_b$}}
\newcommand{\obh}{\mbox{$\Omega_bh^{2}$}}
\newcommand{\om}{\mbox{$\Omega_m$}}
%\newcommand{\ol}{\mbox{$\Omega_{\Lambda } $}}
\newcommand{\sig}{\mbox{$\sigma_8$}}
\newcommand{\gammahe}{\mbox{$\gamma_{228}$}}
\newcommand{\gammah}{\mbox{$\gamma_{912}$}}
\newcommand{\jnu}{\mbox{$J_{\nu }$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Parameters Measured 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\zabs}{\mbox{$z_{\rm abs}$}}
\newcommand{\chisq}{\mbox{$\chi^2$}}
\newcommand{\nhi}{\mbox{N$_{\rm H I}$}}
\newcommand{\lnhi}{\mbox{log \nhi}}
\newcommand{\ndi}{\mbox{N$_{\rm D I}$}}
\newcommand{\lndi}{\mbox{log \ndi}}
\newcommand{\bhi}{\mbox{$b_{\rm H I}$}}
\newcommand{\zdh}{\mbox{$z = 2.526$}}
\newcommand{\zdhvalue}{2.526}
\newcommand{\da}{\mbox{$D_a$}}
\newcommand{\fbar}{\mbox{$\bar{F}$}}
\newcommand{\pdff}{\mbox{flux distribution}}
\newcommand{\bsig}{\mbox{$b_{\sigma}$}}
%\newcommand{\pl}{\mbox{$P_{-2}$}}
\newcommand{\pmed}{\mbox{$P_{-1.5}$}}  
\newcommand{\ps}{\mbox{$P_{-1}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\etal}{{\it et al.}}
\newcommand{\lyaf} {\lya\ forest}
\newcommand{\mf}{\mbox{$10^{-5}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The following defines commands to leave messages in draft copies of the
%% document.  The messages will only be visible if draftmode=true.  
%% \documentclass[11pt,preprint]{aastex}
%% \input{astronomy-commands}
%% \draftmodeptrue  or \draftmodepfalse
%% Note that
%% I use plain old TeX if's instead of Latex's \ifthenelse because the TeX
%% version can be imbedded into Latex commands (such as \section).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifdraftmodep
\draftmodepfalse

\newcommand{\NOTE}[1]{\ifdraftmodep {\color {red} [{\it #1}]} \fi}
\newcommand{\DONE}[1]{\ifdraftmodep {\color {blue} [DONE: {\it #1}]} \fi}
\newcommand{\RESP}[1]{\ifdraftmodep {\color {blue} {\it #1}} \fi}

%\newcommand{\NB}[1]{\ifdraftmodep {\color {red} [NB: {\it #1}]} \fi}
% Rahman Amanullah
\newcommand{\RA}[1]{\ifdraftmodep {\color {red} [RA: {\it #1}]} \fi}
% Kyle Barbary
\newcommand{\KB}[1]{\ifdraftmodep {\color {red} [KB: {\it #1}]} \fi}
% Alex Gude
\newcommand{\AG}[1]{\ifdraftmodep {\color {red} [AG: {\it #1}]} \fi}
% Saul Perlmutter
\newcommand{\SP}[1]{\ifdraftmodep {\color {red} [SP: {\it #1}]} \fi}
% David Rubin
\newcommand{\DR}[1]{\ifdraftmodep {\color {red} [DR: {\it #1}]} \fi}
% Tony Spadafora
\newcommand{\ALS}[1]{\ifdraftmodep {\color {red} [ALS: {\it #1}]} \fi}
% Nao Suzuki
\newcommand{\NS}[1]{\ifdraftmodep {\color {red} [NS: {\it #1}]} \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Define a boolean to indicate if this should be set with emulateapj
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifapjp
\apjpfalse


==> authors_affil.tex <==
\author{ Shadab Alam\altaffilmark{1}}
\author{ Marie Aubert\altaffilmark{2}}
\author{ Santiago Avila\altaffilmark{3,4}}
\author{ Christophe Balland\altaffilmark{5}}
\author{ Julian E. Bautista\altaffilmark{6}}
\author{ Matthew A. Bershady\altaffilmark{7,8,9}}
\author{ Dmitry Bizyaev\altaffilmark{10,11}}
\author{ Michael R.~Blanton\altaffilmark{12}}
\author{ Adam S. Bolton\altaffilmark{13,14}}
\author{ Jo Bovy\altaffilmark{15,16}}
\author{ Jonathan Brinkmann\altaffilmark{10}}
\author{ Joel R.~Brownstein\altaffilmark{14}}
\author{ Etienne Burtin\altaffilmark{17}}
\author{ Sol\`ene Chabanier\altaffilmark{17}}
\author{ Michael J. Chapman\altaffilmark{18,19}}
\author{ Peter Doohyun Choi\altaffilmark{20}}
\author{ Chia-Hsun Chuang\altaffilmark{21}}
\author{ Johan Comparat\altaffilmark{22}}
\author{ Andrei Cuceu\altaffilmark{23}}
\author{ Kyle S. Dawson$^\star$\altaffilmark{14}}
\author{ Axel de la Macorra\altaffilmark{24}}
\author{ Sylvain de la Torre\altaffilmark{25}}
\author{ Arnaud de~Mattia\altaffilmark{17}}
\author{ Victoria de Sainte Agathe\altaffilmark{5}}
\author{ H\'elion~du~Mas~des~Bourboux\altaffilmark{14}}
\author{ Stephanie Escoffier\altaffilmark{2}}
\author{ Thomas Etourneau\altaffilmark{17}}
\author{ James Farr\altaffilmark{23}}
\author{ Andreu Font-Ribera\altaffilmark{26,23}}
\author{ Peter M. Frinchaboy\altaffilmark{27}}
\author{ Sebastien Fromenteau\altaffilmark{28}}
\author{ H\'ector Gil-Mar\'in\altaffilmark{29}}
\author{ Alma X. Gonzalez-Morales\altaffilmark{30,31}}
\author{ Violeta Gonzalez-Perez\altaffilmark{32,6}}
\author{ Kathleen Grabowski\altaffilmark{10}}
\author{ Julien Guy\altaffilmark{33}}
\author{ Adam J. Hawken\altaffilmark{2}}
\author{ Jiamin Hou\altaffilmark{22}}
\author{ Hui Kong\altaffilmark{34}}
\author{ Mark Klaene\altaffilmark{10}}
\author{ Jean-Paul Kneib\altaffilmark{35}}
\author{ Jean-Marc Le Goff\altaffilmark{17}}
\author{ Sicheng Lin\altaffilmark{12}}
\author{ Daniel Long\altaffilmark{10}}
\author{ Brad W. Lyke\altaffilmark{36}}
\author{ Marie-Claude Cousinou\altaffilmark{2}}
\author{ Paul Martini\altaffilmark{37,34}}
\author{ Karen Masters\altaffilmark{38}}
\author{ Faizan G. Mohammad\altaffilmark{18,19}}
\author{ Jeongin Moon\altaffilmark{20}}
\author{ Eva-Maria Mueller$^\star$\altaffilmark{39,6}}
\author{ Andrea Mu\~noz-Guti\'errez\altaffilmark{24}}
\author{ Adam D.~Myers\altaffilmark{36}}
\author{ Seshadri Nadathur\altaffilmark{6}}
\author{ Richard Neveux\altaffilmark{17}}
\author{ Jeffrey A.~Newman\altaffilmark{40}}
\author{ Pasquier Noterdaeme\altaffilmark{41}}
\author{ Audrey Oravetz\altaffilmark{10}}
\author{ Daniel Oravetz\altaffilmark{10}}
\author{ Nathalie Palanque-Delabrouille\altaffilmark{17}}
\author{ Kaike Pan\altaffilmark{10}}
\author{ James Parker III\altaffilmark{10}}
\author{ Romain Paviot\altaffilmark{25}}
\author{ Will J. Percival\altaffilmark{18,19,42}}
\author{ Ignasi P\'erez-R\`afols\altaffilmark{5}}
\author{ Patrick Petitjean\altaffilmark{41}}
\author{ Matthew M. Pieri\altaffilmark{25}}
\author{ Abhishek Prakash\altaffilmark{43}}
\author{ Anand Raichoor\altaffilmark{35}}
\author{ Corentin Ravoux\altaffilmark{17}}
\author{ Mehdi Rezaie\altaffilmark{44}}
\author{ James Rich\altaffilmark{17}}
\author{ Ashley J. Ross\altaffilmark{34}}
\author{ Graziano Rossi\altaffilmark{20}}
\author{ Rossana Ruggeri\altaffilmark{45,6}}
\author{ Vanina Ruhlmann-Kleider\altaffilmark{17}}
\author{ Ariel G. S\'anchez\altaffilmark{22}}
\author{ F.~Javier S\'{a}nchez\altaffilmark{46}}
\author{ Jos\'e R. S\'anchez-Gallego\altaffilmark{47}}
\author{ Conor Sayres\altaffilmark{48}}
\author{ Donald P. Schneider\altaffilmark{49,50}}
\author{ Hee-Jong Seo\altaffilmark{44}}
\author{ Arman Shafieloo\altaffilmark{51,52}}
\author{ An\v{z}e Slosar\altaffilmark{53}}
\author{ Alex Smith\altaffilmark{17}}
\author{ Julianna Stermer\altaffilmark{5}}
\author{ Amelie Tamone\altaffilmark{35}}
\author{ Jeremy L. Tinker\altaffilmark{54}}
\author{ Rita Tojeiro\altaffilmark{55}}
\author{ Mariana Vargas-Maga\~na\altaffilmark{24}}
\author{ Andrei Variu\altaffilmark{35}}
\author{ Yuting Wang\altaffilmark{56}}
\author{ Benjamin A. Weaver\altaffilmark{13}}
\author{ Anne-Marie Weijmans\altaffilmark{55}}
\author{ Christophe Y\`eche\altaffilmark{17}}
\author{ Pauline Zarrouk\altaffilmark{57,17}}
\author{ Cheng Zhao\altaffilmark{35}}
\author{ Gong-Bo Zhao\altaffilmark{56}}
\author{ Zheng Zheng\altaffilmark{14}}
\altaffiltext{1}{\ED}
\altaffiltext{2}{\CPPM}
\altaffiltext{3}{\UAM}
\altaffiltext{4}{\IFT}
\altaffiltext{5}{\LPNHE}
\altaffiltext{6}{\Port}
\altaffiltext{7}{\UWisc}
\altaffiltext{8}{\SAAO}
\altaffiltext{9}{\UCT}
\altaffiltext{10}{\APONMSU}
\altaffiltext{11}{\SAIMSU}
\altaffiltext{12}{\CCPP}
\altaffiltext{13}{\OIRLab}
\altaffiltext{14}{\Utah}
\altaffiltext{15}{\daa}
\altaffiltext{16}{\dunlap}
\altaffiltext{17}{\IRFU}
\altaffiltext{18}{\WCA}
\altaffiltext{19}{\UWaterloo}
\altaffiltext{20}{\Sejong}
\altaffiltext{21}{\KIPAC}
\altaffiltext{22}{\MPE}
\altaffiltext{23}{\UCL}
\altaffiltext{24}{\IFUNAM}
\altaffiltext{25}{\LAM}
\altaffiltext{26}{\IFAE}
\altaffiltext{27}{\TCU}
\altaffiltext{28}{\ICFUNAM}
\altaffiltext{29}{\ICC}
\altaffiltext{30}{\UGTO}
\altaffiltext{31}{\CNCT}
\altaffiltext{32}{\LJMU}
\altaffiltext{33}{\LBL}
\altaffiltext{34}{\CCAPP}
\altaffiltext{35}{\EPFL}
\altaffiltext{36}{\Wyoming}
\altaffiltext{37}{\OSU}
\altaffiltext{38}{\Haverford}
\altaffiltext{39}{\Oxfordastro}
\altaffiltext{40}{\Pitt}
\altaffiltext{41}{\IAP}
\altaffiltext{42}{\PI}
\altaffiltext{43}{\Caltech}
\altaffiltext{44}{\OU}
\altaffiltext{45}{\SUOT}
\altaffiltext{46}{\FNAL}
\altaffiltext{47}{\UWastro}
\altaffiltext{48}{\UW}
\altaffiltext{49}{\PSU}
\altaffiltext{50}{\PSUIGC}
\altaffiltext{51}{\KASSI}
\altaffiltext{52}{\KST}
\altaffiltext{53}{\BNL}
\altaffiltext{54}{\NYU}
\altaffiltext{55}{\StAndrews}
\altaffiltext{56}{\NAOC}
\altaffiltext{57}{\ICCUK}


==> institutionAliases.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                          %
% Institutional aliases file.                              %
% Originally used in CV DM whitepaper,                     %
% successfully stolen for CV 21cm roadmap whitepaper,      %
% now to live a life of its own.                           %
%                                                          %
% When editing, please respect alphabetical ordering       %
% and avoid duplication (that is the entire point).        %
%                                                          %
%                                                          %
% A summer river being crossed                             %
% how pleasing                                             %
% with sandals in my hands!                                %
%       Yosa Buson (1716-1784)                             %
%                                                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Amherst}{University of Massachusetts, Amherst, MA 01003 USA}
\newcommand{\AmsterdamAstro}{Anton Pannekoek Institute for Astronomy, University of Amsterdam, 1098~XH Amsterdam, The Netherlands}
\newcommand{\ANLHEP}{HEP Division, Argonne National Laboratory, Lemont, IL 60439, USA}
\newcommand{\APC}{Laboratoire Astroparticule et Cosmologie (APC), CNRS/IN2P3, Universit\'e Paris Diderot, 10, rue Alice Domon et Léonie Duquet, 75205 Paris Cedex 13, France}
\newcommand{\APONMSU}{Apache Point Observatory and New Mexico State University, P.O. Box 59, Sunspot, NM 88349}
\newcommand{\ASU}{Arizona State University, Tempe, AZ~85287, USA}
\newcommand{\BenGurion}{Department of Physics, Ben-Gurion University, Be'er Sheva 84105, Israel}
\newcommand{\BNL}{Brookhaven National Laboratory, Upton, NY~11973, USA}
\newcommand{\Brown}{Brown University, Providence, RI 02912}
\newcommand{\Bub}{Boston University, Boston, MA 02215}
\newcommand{\BU}{Boston University, Boston, MA 02215}
\newcommand{\Buffalo}{Department of Physics, University at Buffalo, SUNY Buffalo, NY 14260 USA}
\newcommand{\Caltech}{California Institute of Technology, Pasadena, CA 91125}
\newcommand{\Cardiff}{School of Physics and Astronomy, Cardiff University, The Parade, Cardiff, CF24 3AA, UK}
\newcommand{\Carleton}{Carleton University, K1S 5B6 Ottawa, Canada}
\newcommand{\Carnegie}{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara St., Pasadena, CA 91101, USA}
\newcommand{\Cavendish}{Astrophysics Group, Cavendish Laboratory, J.J.Thomson Avenue, Cambridge, CB3 0HE, UK}
\newcommand{\CCA}{Center for Computational Astrophysics, Flatiron Institute, New York, NY~10010, USA}
\newcommand{\CCAPP}{Center for Cosmology and AstroParticle Physics, The Ohio State University, Columbus, OH 43212}
\newcommand{\CCPP}{Center for Cosmology and Particle Physics, Department of Physics, New York University, 726 Broadway, Room 1005, New York, NY 10003, USA}
\newcommand{\CPPM}{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}
\newcommand{\CEADAP}{D\'epartement d’Astrophysique, CEA Saclay DSM/Irfu, 91191 Gif-sur-Yvette, France}
\newcommand{\CERN}{CERN, Geneva, Switzerland}
\newcommand{\CfA}{Harvard-Smithsonian Center for Astrophysics, MA 02138}
\newcommand{\CFT}{Center for Theoretical Physics, Polish Academy of Sciences, al. Lotnik\'{o}w 32/46, 02-668, Warsaw, Poland}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH 45221}
\newcommand{\CITA}{Canadian Institute for Theoretical Astrophysics, University of Toronto, Toronto, ON~M5S~3H8, Canada}
\newcommand{\CNRSA}{CNRS, Laboratoire d'Annecy-le-Vieux de Physique Th\'{e}orique, France}
\newcommand{\CNYang}{C.N.\ Yang Institute for Theoretical Physics, State University of New York Stony Brook, NY~11794, USA}
\newcommand{\CNCT}{Consejo Nacional de Ciencia y Tecnolog\'ia, Av. Insurgentes Sur 1582. Colonia Cr\'edito Constructor, Del. Benito Ju\'arez, C.P. 03940, M\'exico D.F. M\'exico}
\newcommand{\CMUCosmo}{Department of Physics, McWilliams Center for Cosmology, Carnegie Mellon University}
\newcommand{\Columbia}{Columbia University, New York, NY 10027}
\newcommand{\Cornell}{Cornell University, Ithaca, NY~14853, USA}
\newcommand{\CPthree}{CP3-Origins, 5230 Odense, Denmark}
\newcommand{\CUBoulder}{Center for Astrophysics and Space Astronomy, Department of Astrophysical and Planetary Science, University of Colorado, Boulder, CO 80309, USA}
\newcommand{\CWRU}{Case Western Reserve University, Cleveland, OH 44106}
\newcommand{\daa}{Department of Astronomy and Astrophysics, University of Toronto, ON, M5S3H4}
\newcommand{\damtp}{DAMTP, Centre for Mathematical Sciences, Wilberforce Road, Cambridge, UK, CB3 0WA}
\newcommand{\DESY}{DESY,  22607 Hamburg, Germany}
\newcommand{\dfa}{Departamento de F\'{\i}sica e Astronomia, Faculdade de Ci\^{e}ncias, Universidade do Porto, Porto, Portugal}
\newcommand{\DFI}{Departamento de F\'isica, FCFM, Universidad de Chile, Blanco Encalada 2008, Santiago, Chile}
\newcommand{\DOE}{US. Department of Energy, Germantown, MD 20874}
\newcommand{\drexel}{Drexel University, Philadelphia, PA 19104}
\newcommand{\Duke}{Duke University and Triangle Universitites Nuclear Laboratory, Durham, NC 27708}
\newcommand{\DukePhys}{Department of Physics, Duke University, Durham, NC 27708, USA}
\newcommand{\dunlap}{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, ON~M5S~3H4, Canada}
\newcommand{\Durham}{Department of Physics, Lower Mountjoy, South Rd, Durham DH1 3LE, United Kingdom}
\newcommand{\ED}{University of Edinburgh, Edinburgh EH8~9YL, UK}
\newcommand{\EPFL}{Institute of Physics, Laboratory of Astrophysics, Ecole Polytechnique Fédérale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland}
\newcommand{\ETH}{ETH Zurich, Institute for Particle Physics, 8093 Zurich, Switzerland}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL~60510, USA}
\newcommand{\FQAUB}{Dept. de F\' isica Qu\` antica i Astrof\' isica, Universitat de Barcelona, Mart\' i i Franqu\` es 1, E08028 Barcelona, Spain}
\newcommand{\FSU}{Florida State University, Tallahassee, FL 32306}
\newcommand{\Glasgow}{University of Glasgow, G12 8QQ Glasgow, United Kingdom}
\newcommand{\GRAPPA}{GRAPPA Institute, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
\newcommand{\GSFC}{Goddard Space Flight Center, Greenbelt, MD 20771 USA}
\newcommand{\GWU}{George Washington University, Washington, DC 20052}
\newcommand{\Hampton}{Hampton University, Hampton, VA 23668}
\newcommand{\HarvardPhys}{Department of Physics, Harvard University, Cambridge, MA~02138, USA}
\newcommand{\Haverford}{Haverford College, 370 Lancaster Ave, Haverford PA, 19041, USA}
\newcommand{\Hawaii}{University of Hawaii, Honolulu, HI 96822}
\newcommand{\HKUST}{The Hong Kong University of Science and Technology, Hong Kong SAR, China}
\newcommand{\houston}{University of Houston, Houston, TX 77204}
\newcommand{\IA}{Instituto de Astrof\'{\i}sica e Ci\^encias do Espa\c{c}o (IA), Porto, Portugal}
\newcommand{\IAC}{Instituto de Astrof\'{\i}sica de Canarias, 38200 La Laguna, Tenerife, Spain}
\newcommand{\IAP}{Institut d'Astrophysique de Paris, CNRS \& Sorbonne University, UMR 7095, 98bis bd Arago, 75014 Paris, France}
\newcommand{\IAS}{Institute for Advanced Study, Princeton, NJ~08540, USA}
\newcommand{\IBS}{Institute for Basic Science (IBS), Daejeon 34051, Korea}
\newcommand{\ICC}{ICC, University of Barcelona, IEEC-UB, Mart\' i i Franqu\` es, 1, E08028 Barcelona, Spain}
\newcommand{\ICCD}{Institute for Computational Cosmology, Department of Physics, Durham University, South Road, Durham, DH1 3LE, UK}
\newcommand{\ICCUK}{Institute for Computational Cosmology, Dept. of Physics, Univ. of Durham, South Road, Durham DH1 3LE, UK}
\newcommand{\ICE}{Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, 08193 Barcelona, Spain}
\newcommand{\ICFUNAM}{ICFUNAM - Instituto de Ciencias F\'{i}sicas, Universidad Nacional Aut\'onoma de M\'exico,  62210 Cuernavaca, Mor., M\'exico}
\newcommand{\ICRR}{Institute for Cosmic Ray Resaerch, The University of Tokyo, 456 Higashi-Mozumi, Kamioka, Hida, Gifu 506-1205, Japan}
\newcommand{\ICTP}{International Centre for Theoretical Physics, Strada Costiera, 11, I-34151 Trieste, Italy}
\newcommand{\IFAE}{Institut de F\'{i}sica d’Altes Energies, The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona), Spain}
\newcommand{\IFPU}{IFPU - Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy}
\newcommand{\IFT}{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\newcommand{\IFUNAM}{IFUNAM - Instituto de F\'{i}sica, Universidad Nacional Aut\'onoma de M\'exico, 04510 CDMX, M\'exico}
\newcommand{\IHEP}{Institute of High Energy Physics, Austrian Academy of Sciences, 1050 Vienna, Austria}
\newcommand{\Imperial}{Theoretical Physics, Blackett Laboratory, Imperial College, London, SW7 2AZ, U.K.}
\newcommand{\Indiana}{Indiana University, Bloomington, IN 47405}
\newcommand{\INAFOATs}{INAF - Osservatorio Astronomico di Trieste, Via G.B. Tiepolo 11, 34143 Trieste, Italy}
\newcommand{\INAFOAS}{INAF - Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, via Piero Gobetti 93/3, I-40129 Bologna, Italy}
\newcommand{\INFNCag}{Istituto Nazionale di Fisica Nucleare, Sezione di Cagliari,  09126 Cagliari, Italy}
\newcommand{\INFNCat}{Istituto Nazionale di Fisica Nucleare, Sezione di Catania, 95125 Catania, Italy}
\newcommand{\INFNG}{Istituto Nazionale di Fisica Nucleare, Sezione di Genova, 16146 Genova, Italy}
\newcommand{\INFN}{INFN – National Institute for Nuclear Physics, Via Valerio 2, I-34127 Trieste, Italy}
\newcommand{\INFNFE}{Istituto Nazionale di Fisica Nucleare, Sezione di Ferrara, 40122, Italy }
\newcommand{\INFNLNF}{Istituto Nazionale di Fisica Nucleare, Laboratori Nazionali di Frascati, 00044 Frascati, Italy}
\newcommand{\INFNLNS}{Istituto Nazionale di Fisica Nucleare, Laboratori Nazionali del Sud, 95125 Catania, Italy}
\newcommand{\INFNN}{Istituto Nazionale di Fisica Nucleare, Sezione di Napoli, 80125 Napoli, Italy }
\newcommand{\INFNPD}{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, 35131~Padova, Italy}
\newcommand{\INFNRM}{Istituto Nazionale di Fisica Nucleare, Sezione di Roma, 00185 Roma, Italy}
\newcommand{\INFNT}{Istituto Nazionale di Fisica Nucleare, Sezione di Torino, 10125, Italy }
\newcommand{\ioa}{Institute of Astronomy, University of Cambridge,Cambridge CB3 0HA, UK}
\newcommand{\IPP}{Institute for Particle Physics, BC V8W 3P6 Victoria, Canada}
\newcommand{\IPMU}{Kavli Institute for the Physics and Mathematics of the Universe, University of Tokyo, Kashiwa, Japan}
\newcommand{\IPNL}{Universit\'e de Lyon, F-69622, Lyon, France; Universit\'e de Lyon 1, Villeurbanne; CNRS/IN2P3, Institut de Physique Nucl\'eaire de Lyon}
\newcommand{\IRFU}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\newcommand{\ITFA}{Institute for Theoretical Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
\newcommand{\IUCAA}{The Inter-University Centre for Astronomy and Astrophysics, Pune, 411007, India}
\newcommand{\Jerusalem}{Hebrew University of Jerusalem, 91904 Jerusalem, Israel}
\newcommand{\JHU}{Johns Hopkins University, Baltimore, MD 21218}
\newcommand{\JLAB}{Thomas Jefferson National Laboratory, Newport News, VA 23606}
\newcommand{\JPL}{Jet Propulsion Laboratory, California Institute of Technology, Pasadena, CA, USA}
\newcommand{\KASSI}{Korea Astronomy and Space Science Institute, Daejeon 34055, Korea}
\newcommand{\kavli}{Kavli Institute for Cosmology, Cambridge, UK, CB3 0HA}
\newcommand{\KIAS}{School of Physics, Korea Institute for Advanced Study, 85 Hoegiro, Dongdaemun-gu, Seoul 130-722, Korea}
\newcommand{\KICP}{Kavli Institute for Cosmological Physics, Chicago, IL 60637}
\newcommand{\KIPAC}{Kavli Institute for Particle Astrophysics and Cosmology, Stanford 94305}
\newcommand{\KINGS}{King's College London, WC2R 2LS London, United Kingdom}
\newcommand{\Kobe}{Kobe University, 657-8501 Kobe, Japan}
\newcommand{\KPH}{Johannes Gutenberg University, 55128 Mainz, Germany}
\newcommand{\KPMU}{University of Tokyo, 277-8583  Kashiwa , Japan}
\newcommand{\KST}{University of Science and Technology, Daejeon 34113, Korea}
\newcommand{\KSU}{Kansas State University, Manhattan, KS 66506}
\newcommand{\KwaZuluNatal}{Astrophysics and Cosmology Research Unit, School of Chemistry and Physics, University of KwaZulu-Natal, Durban 4000, South Africa}
\newcommand{\Lafayette}{Lafayette College, Easton, PA 18042}
\newcommand{\LANL}{Los Alamos National Laboratory, Los Alamos, NM 87545}
\newcommand{\LBL}{Lawrence Berkeley National Laboratory, Berkeley, CA~94720, USA}
\newcommand{\Leiden}{Lorentz Institute, Leiden University, Niels Bohrweg 2,Leiden, NL 2333 CA, The Netherlands}
\newcommand{\Liverpool}{University of Liverpool,  L69 7ZE Liverpool , United Kingdom}
\newcommand{\LJMU}{Liverpool John Moores University,  L3 5RF Liverpool , United Kingdom}
\newcommand{\LLNL}{Lawrence Livermore National Laboratory, Livermore, CA, 94550}
\newcommand{\LPC}{Universit\'e Clermont Auvergne, CNRS/IN2P3, Laboratoire de Physique de Clermont, F-63000 Clermont-Ferrand, France}
\newcommand{\LPNHE}{Sorbonne Universit\'e, Universit\'e Paris Diderot, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies, LPNHE, 4 Place Jussieu, F-75252 Paris, France}
\newcommand{\McGill}{McGill University, Montreal, QC~H3A~2T8, Canada}
\newcommand{\Melbourne}{School of Physics, The University of Melbourne, Parkville, VIC 3010, Australia}
\newcommand{\Mines}{Colorado School of Mines, Golden, CO 80401}
\newcommand{\MIT}{Massachusetts Institute of Technology, Cambridge, MA 02139}
\newcommand{\MPE}{Max-Planck-Institut f\"{u}r extraterrestrische Physik (MPE), Giessenbachstrasse 1, D-85748 Garching bei M\"unchen, Germany}
\newcommand{\MPIA}{Max-Planck-Institut f\"{u}r Astrophysik, Karl-Schwarzschild-Str. 1, 85741 Garching, Germany}
\newcommand{\MPP}{Max-Planck-Institut f\"{u}r Physik (Werner-Heisenberg-Institut), F\"ohringer Ring 6, D-80805 M\"unchen, Germany}
\newcommand{\LAM}{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France}
\newcommand{\LUPM}{Laboratoire Univers et Particules de Montpellier, Univ. Montpellier and CNRS, 34090 Montpellier, France}
\newcommand{\NAOC}{National Astronomical Observatories of China, Chinese Academy of Sciences, 20A Datun Road, Chaoyang District, Beijing 100012, China}
\newcommand{\NCBJ}{National Center for Nuclear Research, Ul.Pasteura 7,Warsaw, Poland}
\newcommand{\NCU}{National Central University, Taoyuan City 32001, Taiwan (R.O.C.)}
\newcommand{\NCSU}{Physics Department, North Carolina State Universitym, 2401 Stinson Dr, Raleigh, NC 27607}
\newcommand{\ND}{University of Notre Dame,vNotre Dame, IN 46556}
\newcommand{\NIU}{Northern Illinois University, DeKalb, Illinois 60115}
\newcommand{\NMSU}{New Mexico State University, Las Cruces, NM 88003}
\newcommand{\NOAO}{National Optical Astronomy Observatory, 950 N. Cherry Ave., Tucson, AZ 85719 USA}
\newcommand{\Northwestern}{Northwestern University, Evanston, IL 60201}
\newcommand{\Nottingham}{University of Nottingham, NG7 2RD Nottingham, United Kingdom}
\newcommand{\NPPSFAmes}{NASA Postdoctoral Program Senior Fellow, NASA Ames Research Center, Moffett Field, CA 94035, USA}
\newcommand{\NWU}{Northwestern University, Evanston, IL 60208}
\newcommand{\NYU}{New York University, New York, NY 10003}
\newcommand{\OIRLab}{NSF's National Optical-Infrared Astronomy Research Laboratory, 950 N. Cherry Ave, Tucson, AZ 85719 USA}
\newcommand{\OK}{ University of Oklahoma, Norman, OK 73019}
\newcommand{\ORNL}{Oak Ridge National Laboratory, Oak Ridge, TN 37831}
\newcommand{\OSU}{The Ohio State University, Columbus, OH 43212}
\newcommand{\OU}{Department of Physics and Astronomy, Ohio University, Clippinger Labs, Athens, OH 45701, USA}
\newcommand{\OskarKlein}{Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm SE-106 91, Sweden}
\newcommand{\Oxford}{University of Oxford, Oxford OX1~3RH, UK}
\newcommand{\Oxfordastro}{Sub-department of Astrophysics, Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH}
\newcommand{\Oxy}{Occidental College, Los Angeles, CA 90041}
\newcommand{\ParisSud}{Universit\'{e} Paris-Sud, LAL, UMR 8607, F-91898 Orsay Cedex, France \& CNRS/IN2P3, F-91405 Orsay, France}
\newcommand{\PI}{Perimeter Institute, Waterloo, ON~N2L~2Y5, Canada}
\newcommand{\Pitt}{University of Pittsburgh and PITT PACC, Pittsburgh, PA 15260}
\newcommand{\PNNL}{Pacific Northwest National Laboratory ,Richland, WA 99352}
\newcommand{\PNPI}{Petersburg Nuclear Physics Institute, 188300 Gatchina, Russia}
\newcommand{\Port}{Institute of Cosmology \& Gravitation, University of Portsmouth, Dennis Sciama Building, Burnaby Road, Portsmouth PO1 3FX, UK}
\newcommand{\Princeton}{Princeton University, Princeton, NJ 08544}
\newcommand{\PSU}{The Pennsylvania State University, University Park, PA 16802}
\newcommand{\PSUAstro}{Department of Astronomy and Astrophysics, The Pennsylvania State University, University Park, PA 16802}
\newcommand{\PSUIGC}{Institute for Gravitation and the Cosmos, The Pennsylvania State University, University Park, PA 16802}
\newcommand{\Purdue}{Purdue University, West Lafayette, IN 47907}
\newcommand{\PW}{Participation Worldscope, Sedona, Arizona and Hong Kong, SAR PRC}
\newcommand{\Queens}{Queen's University , K7L 3N6 Kingston, Canada}
\newcommand{\Queensland}{The University of Queensland, School of Mathematics and Physics, QLD 4072, Australia}
\newcommand{\QMUL}{Queen Mary University of London, London E1~4NS, UK}
\newcommand{\RAL}{Radio Astronomy Laboratory, University of California Berkeley, Berkeley, CA 94720, USA}
\newcommand{\Rice}{Department of Physics \& Astronomy, Rice University, Houston, Texas 77005, USA}
\newcommand{\RIT}{Rochester Institute of Technology}
\newcommand{\RomaS}{Dipartimento di Fisica, Universit\`{a} La Sapienza, P. le A. Moro 2, Roma, Italy}
\newcommand{\RUG}{Kapteyn Astronomical Institute, University of Groningen, P.O. Box 800, 9700 AV Groningen, The Netherlands}
\newcommand{\Rutgers}{Department of Physics and Astronomy, Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854, USA}
\newcommand{\SAAO}{South African Astronomical Observatory, PO Box 9, Observatory 7935, Cape Town, South Africa}
\newcommand{\SAIMSU}{Sternberg Astronomical Institute, Moscow State University, Moscow, 119992, Russia}
\newcommand{\Sanford}{Sanford Underground Research Facility, Lead, SD 57754}
\newcommand{\Sassari}{Universit\`a di Sassari, 07100 Sassari,  Italy}
\newcommand{\SCIPP}{University of California at Santa Cruz, Santa Cruz, CA 95064; USA}
\newcommand{\Sejong}{Department of Physics and Astronomy, Sejong University, Seoul, 143-747, Korea}
\newcommand{\Sheffield}{University of Sheffield, S3 7RH Sheffield, United Kingdom}
\newcommand{\SHAO}{Shanghai Astronomical Observatory (SHAO), Nandan Road 80, Shanghai 200030, China}
\newcommand{\Siena}{Siena College, 515 Loudon Road, Loudonville, NY 12211, USA}
\newcommand{\SISSA}{SISSA - International School for Advanced Studies, Via Bonomea 265, 34136 Trieste, Italy}
\newcommand{\SimonFraser}{Department of Physics, Simon Fraser University, Burnaby, British Columbia, Canada V5A 1S6}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
\newcommand{\SMU}{Southern Methodist University, Dallas, TX 75275}
\newcommand{\SNOLAB}{SNOLAB, Lively, ON P3Y 1N2, Canada}
\newcommand{\SoCal}{University of Southern California, CA 90089 }
\newcommand{\StAndrews}{School of Physics and Astronomy, University of St Andrews, North Haugh, St Andrews, KY16 9SS, UK}
\newcommand{\Stanford}{Stanford University, Stanford, CA 94305}
\newcommand{\StonyBrook}{Stony Brook University, Stony Brook, NY~11794, USA}
\newcommand{\STSCI}{Space Telescope Science Institute, Baltimore, MD 21218}
\newcommand{\SUNYA}{University at Albany SUNY, Albany, NY 12222}
\newcommand{\SUOT}{Swinburne University of Technology, Centre for Astrophysics and Supercomputing, Melbourne, VIC 3122, Australia}
\newcommand{\SussexAstronomy}{Astronomy Centre, School of Mathematical and Physical Sciences, University of Sussex, Brighton BN1 9QH, United Kingdom}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY 13244}
\newcommand{\Tamu}{Texas AandM University, College Station, TX 77843 }
\newcommand{\TCU}{Department of Physics \& Astronomy, Texas Christian University, Fort Worth, TX 76129, USA}
\newcommand{\Techsource}{Techsource Incorporated, Los Alamos, NM 87544}
\newcommand{\TelAviv}{Tel-Aviv University,  69978 Tel-Aviv, Israel}
\newcommand{\Temple}{Temple University, Philadelphia, PA 19122}
\newcommand{\TIFR}{Tata Institute of Fundamental Research, Homi Bhabha Road, Mumbai 400005 India}
\newcommand{\Tsinghua}{Department of Physics and Tsinghua Center for Astrophysics, Tsinghua University, Beijing 100084, P R China}
\newcommand{\TUM}{Technical University of Munich,  80333 Munich, Germany}
\newcommand{\UA}{University of Alabama, Tuscaloosa, AL 35487}
\newcommand{\UAS}{Department of Astronomy/Steward Observatory, University of Arizona, Tucson, AZ  85721}
\newcommand{\UAM}{Universidad Aut\'onoma de Madrid, 28049, Madrid, Spain}
\newcommand{\UBC}{University of British Columbia, Vancouver, BC V6T 1Z1, Canada}
\newcommand{\UCB}{Department of Astronomy, University of California Berkeley, Berkeley, CA~94720, USA}
\newcommand{\UCBP}{Department of Physics, University of California Berkeley, Berkeley, CA~94720, USA}
\newcommand{\UCBSSL}{Space Sciences Laboratory, University of California Berkeley, Berkeley, CA 94720, USA}
\newcommand{\UCD}{University of California at Davis, Davis, CA 95616}
\newcommand{\UChicago}{University of Chicago, Chicago, IL 60637}
\newcommand{\UCI}{University of California, Irvine, CA 92697}
\newcommand{\UCLA}{University of California at Los Angeles, Los Angeles,  CA 90095}
\newcommand{\UCL}{University College London, WC1E 6BT London, United Kingdom}
\newcommand{\UCR}{University of California at Riverside, Riverside, CA 92521}
\newcommand{\UCSB}{University of California at Santa Barbara, Santa Barbara, CA 93106}
\newcommand{\UCSC}{University of California Santa Cruz, Santa Cruz, CA~95064, USA}
\newcommand{\UCSD}{University of California San Diego, La Jolla, CA~92093, USA}
\newcommand{\UCT}{Department of Astronomy, University of Cape Town, Private Bag X3, Rondebosch 7701, South Africa}
\newcommand{\UFL}{University of Florida, Gainesville, FL 32611}
\newcommand{\UFN}{Universit\`a Federico II di Napoli, 80125 Napoli, Italy}
\newcommand{\UGTO}{Divisi\'on de Ciencias e Ingenier\'ias, Universidad de Guanajuato, Le\'on 37150, M\'exico}
\newcommand{\UKY}{University of Kentucky, Lexington, KY 40506}
\newcommand{\UMD}{University of Maryland, College Park, MD 20742
\newcommand{\UMiami}{University of Miami, Coral Gables, FL 33124}}
\newcommand{\UMich}{University of Michigan, Ann Arbor, MI 48109}
\newcommand{\UMN}{University of Minnesota, Minneapolis, MN 55455}
\newcommand{\UnB}{Instituto de F\'{i}sica, Universidade de Bras\'{i}lia, 70919-970, Bras\'{i}lia, DF, Brazil}
\newcommand{\UNC}{University of North Carolina at Chapel Hill, Chapel Hill, NC 27599}
\newcommand{\UNH}{University of New Hampshire, Durham, NH 03824}
\newcommand{\UNIMI}{Dipartimento di Fisica ``Aldo Pontremoli'', Universit\`a{} degli Studi di Milano, via Celoria 16, 20133 Milano, Italy}
\newcommand{\UNIPD}{Dipartimento di Fisica e Astronomia ``G. Galilei'', Universit\`a degli Studi di Padova, 35131~Padova, Italy}
\newcommand{\UNM}{University of New Mexico, Albuquerque, NM 87131}
\newcommand{\UNV}{University of Nevada, Reno, NV 89557}
\newcommand{\UoM}{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
\newcommand{\UPenn}{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\newcommand{\UR}{Department of Physics and Astronomy, University of Rochester, 500 Joseph C. Wilson Boulevard, Rochester, NY 14627, USA}
\newcommand{\UrbanaC}{Department of Physics, University of Illinois at Urbana-Champaign, Urbana, IL~61801, USA}
\newcommand{\USC}{The University of South Carolina, Columbia, SC 29208}
\newcommand{\USD}{The University of South Dakota, Vermillion, SD 57069}
\newcommand{\UTD}{University of Texas at Dallas, Texas 75080}
\newcommand{\Utenn}{The University of Tennessee, Knoxville, TN 37996}
\newcommand{\Utah}{University of Utah, Department of Physics and Astronomy, 115 S 1400 E, Salt Lake City, UT 84112, USA}
\newcommand{\UVA}{University of Virginia, Charlottesville, VA 22903}
\newcommand{\Uvic}{University of Victoria, BC V8P 5C2 Victoria, Canada}
\newcommand{\UWaterloo}{Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}
\newcommand{\UWisc}{Department of Astronomy, University of Wisconsin-Madison, Madison, WI~53706, USA}
\newcommand{\UWMadison}{Department of Physics, University of Wisconsin-Madison, Madison, WI~53706, USA}
\newcommand{\UW}{University of Washington, Seattle 98195}
\newcommand{\UWastro}{Department of Astronomy, University of Washington, Box 351580, Seattle, WA 98195, USA}
\newcommand{\UWC}{Department of Physics \& Astronomy, University of the Western Cape, Cape Town 7535, South Africa}
\newcommand{\Vanderbilt}{Physics \& Astronomy Department, Vanderbilt University, PMB 401807, 2301 Vanderbilt Place, Nashville, TN 37235}
\newcommand{\VSI}{Van Swinderen Institute for Particle Physics and Gravity, University of Groningen, 9747~AG~Groningen, The~Netherlands}
\newcommand{\VT}{Virginia Tech, Blacksburg, VA 24061}
\newcommand{\VUU}{Virginia Union University, Richmond, Virginia, 23220}
\newcommand{\WCA}{Waterloo Centre for Astrophysics, University of Waterloo, Waterloo, ON~N2L~3G1, Canada} 
\newcommand{\Weizmann}{Weizmann Institute of Science, 76100 Rehovot, Israel}
\newcommand{\Wellesley}{Wellesley College, Wellesley, MA 02481}
\newcommand{\wiscIce}{University of Wisconsin, Madison, WI 53706}
\newcommand{\WM}{College of William and Mary, Newport News, VA 23606}
\newcommand{\WUSL}{Washington University in St Louis, St. Louis, MO 63130}
\newcommand{\WVU}{CSEE, West Virginia University, Morgantown, WV 26505, USA}
\newcommand{\WVUGWAC}{Center for Gravitational Waves and Cosmology, West Virginia University, Morgantown, WV 26505, USA}
\newcommand{\Wyoming}{Department of Physics and Astronomy, University of Wyoming, Laramie, WY 82071, USA}
\newcommand{\Yale}{Department of Physics, Yale University, New Haven, CT~06520, USA}
\newcommand{\YorkU}{Department of Physics and Astronomy, York University, Toronto, ON~M3J~1P3, Canada}

